Font Representation Learning via Paired-glyph Matching

Fonts can convey profound meanings of words in various forms of glyphs. Without typography knowledge, manually selecting an appropriate font or designing a new font is a tedious and painful task. To allow users to explore vast font styles and create new font styles, font retrieval and font style transfer methods have been proposed. These tasks increase the need for learning high-quality font representations. Therefore, we propose a novel font representation learning scheme to embed font styles into the latent space. For the discriminative representation of a font from others, we propose a paired-glyph matching-based font representation learning model that attracts the representations of glyphs in the same font to one another, but pushes away those of other fonts. Through evaluations on font retrieval with query glyphs on new fonts, we show our font representation learning scheme achieves better generalization performance than the existing font representation learning techniques. Finally on the downstream font style transfer and generation tasks, we confirm the benefits of transfer learning with the proposed method. The source code is available at https://github.com/junhocho/paired-glyph-matching.

==> debug_notes.tex <==

\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Method                                          & MSE                   & Notes \\
\hline\hline
                                                & 10.50 (10.25)               & AE \\
NKN (CVPR'18)~\cite{villegas2018neural}         & \textbf{7.68} (8.51)       & Cycle \\
                                                & 8.87 (7.10)                  & Cycle + Adv \\
\hline
\hline
Copy                                           & 9.00                  & Copy input quaternions and velocities \\
\hline
\hline
0326                                            & 9.20                  & v3 \\
\hline
\hline
0404                                            & 346.66                & \\
0404 b                                          & 9.50                  &  \\
0404 gr                                         & 9.18                  &  \\
0405 L1reg                                      & 9.17                  & v4\\
0405 L1reg 0.1b                                 & \textbf{6.62}         &  \\
0405 L1reg 1b                                   & 7.04                  & \\
0405 L2reg 1b                                   & 12.49                 & \\
0405 NOreg 1b                                   & 237.62                & \\
\hline
\hline
0409 L1 0.1b                                    & 6.20                  & \\
0410 L1 1b                                      & \textbf{5.84}         & \\
0410 L1 5b                                      & 6.28                  & v5(only mul global motion) \\
0410 L2 1b                                      & 10.28                 & \\
\hline
0410 L2 1b                                     & 3.63                  & no activation in last layer \\
0411 L1 1b                                     & 3.74                  &  \\
0412 L2 5b                                     & \textbf{2.72}         &  \\
0412 L1 5b both                                & 3.82                  &  global ae L1 \\
0413 L2 5b noadv                               & 3.57                  &  no adv, only reg \\
0414 L2 5b noreg                               & 11.54                  &  only adv \\
\hline\hline
0415 v6                                        & 5.04                  & 5*L2 reg, 1*ground contact adv \\
0416 v6.1 bug fix                              & 6.31                  & 5*L2 reg, 1*mean/h adv, bugfix \\
\hline\hline
0417 v7                                        & 2.59                  & 1reg,1b! \\
0417 v7.1                                      & \textbf{2.43}         & 5reg:1b, ae도 normalized \\
0417 v7.1 noadv                                & 2.58                  & 5reg:noadv! \\
0418 v7 0.1b                                   & 2.52                  & 5reg:0.1b \\
0418 v7 5b1reg                                 & 2.55                  & 1reg:5b \\
0418 v7 5b noreg                               & -.--                  & noreg:5b \\
\hline
\hline
0418 v8 1b5r1s                                & 2.56                & shape L2 \\
0420 v8 1b5r0.1s                              & 2.52                & shape disc \\
\hline
드디어! &\textbf{2.38} & xyz mean, 0.001 슬슬 실험 정리하자.\\
\hline
\end{tabular}
\end{center}
\caption{Debug notes...}
\end{table}

==> figure/fig-anatomy-of-typography.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{image/anatomy-of-typography.png}
  \caption{
  Anatomy of typography. Designing font requires professional knowledge of typography.
  }
%   \Description{Anatomy of typography.}
  \label{fig:anatomy-of-typography}
\end{figure}


==> figure/fig-character-retireval-accuracy.tex <==
\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{image/char-retrieval-accuracy.png}
  \caption{
  Retrieval accuracy for each characters.
  Ex) (G $\rightarrow$ R) : From each embeddings of ``G'' of 28 different fonts, retrieve the closest embedding ``R'' and check if ``R'' belongs to same font of ``G''.
  }
%   \Description{Retrieval accuracy for each characters.}
  \label{fig:character-retrieval-accuracy}
\end{figure}


==> figure/fig-downstream-attr2font.tex <==
\begin{figure}[]
  \centering
  \includegraphics[width=0.93\linewidth]{image/downstream-attr2font.pdf}
  \vspace{-0.8cm}
  \caption{
  Attr2Font~\cite{WangSIGGRAPH2020} performance ($\texttt{L1-error}$) with the \textcolor{teal}{OFL dataset pretrained} and \textcolor{gray}{random} initialization.
  }
%   \Description{Font style transfer task performance.}
  \label{fig:downstream-attr2font}
  \vspace{-0.5cm}

\end{figure}


==> figure/fig-functions.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{image/functions.png}
  \caption{
  Functions in our model.
  }
%   \Description{Functions in our model.}
  \label{fig:functions}
\end{figure}


==> figure/fig-glyphs-in-a-font.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.5\linewidth]{image/glyphs-in-a-font.pdf}
  \caption{
  Glyphs in each font.
  }
%   \Description{Glyphs in each font.}
  \label{fig:glyphs-in-a-font}
\end{figure}


==> figure/fig-ofl-embeddings.tex <==
\begin{figure*}[]\centering
\includegraphics[width=0.8\linewidth]{image/ofl_embedding.pdf}
\caption{Font latent space of the OFL dataset annotated by font classes and character classes for each embedding methods.
} 
% \Description{Font Embedding Methods}
\label{fig:ofl-embeddings}
\end{figure*}



==> figure/fig-retrieval-accuracy-attribute-learning-per-samples.tex <==
% fig:retrieval-accuracy-on-validation-set
\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{image/fig-attribute-learning-per-samples.png}
  \caption{
    Retrieval Accuracy on Validation Set. Each experiment shows different samples of none attribute annotated fonts for unsupervised learning. This indicates that lack of data for unsupervised learning leads to overfitting.
    \rev{Figure 수정 필요하면 수정.}
  }
%   \Description{}
  \label{fig:retrieval-accuracy-attribute-learning-per-samples}
\end{figure}


==> figure/fig-retrieval-accuracy-on-validation-set.tex <==
% fig:retrieval-accuracy-on-validation-set
\begin{figure}[]
  \centering
  \includegraphics[width=\linewidth]{image/retrieval-accuracy-on-validation-set.png}
  \caption{
    Retrieval Accuracy on Validation Set.
    \rev{Revise after training, Include autoencoder.}
    This indicates \rev{glyph autoencoder is poor}, font classification models easily overfit, while proposed method is robust on feature learning of fonts.
  }
%   \Description{}
  \label{fig:retrieval-accuracy-on-validation-set}
\end{figure}


==> figure/fig-supplementary_capitals_to_donovan_attributes.tex <==

\begin{figure*}[]\centering
\includegraphics[width=1\linewidth]{image/supp_capitals_to_donovan_attributes.pdf}
\vspace*{-0.5cm}
\caption{Font latent space on the O'Donovan dataset annotated by font  attributes.
} 
% \Description{Font Embedding Methods with attributes}
\label{fig:supplementary_capitals_to_donovan_attributes}
\vspace{-0.5cm}
\end{figure*}



==> figure/fig-supplementary_capitals_to_donovan_classes.tex <==

\begin{figure*}[]\centering
\includegraphics[width=0.92\linewidth]{image/supp_capitals_to_donovan_classes.pdf}
\vspace*{-0.3cm}
\caption{Font latent space on the O'Donovan dataset annotated by font and character classes.
} 
% \Description{Font Embedding Methods with attributes}
\label{fig:supplementary_capitals_to_donovan_classes}
\vspace{-0.3cm}
\end{figure*}



==> figure/fig-supplementary_linear_evaluation_protocol.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{image/supp_linear_eval.pdf}
  \vspace{-0.8cm}
  \caption{
  Font attribute prediction results from $\hat{f}$ of each method.
  }
%   \Description{Anatomy of typography.}
  \label{fig:supplementary-linear-evaluation-protocol}
\end{figure}


==> figure/fig-supplementary_loss_function.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\linewidth]{image/supp_loss_h.pdf}
  \caption{
  Detailed description on the loss function of {\it Paired-glyph Matching} learning.
  }
%   \Description{Detailed description on the loss function of {\it Paired-glyph Matching} learning. }
  \label{fig:supplementary_loss_fuction}
\end{figure}


==> figure/fig-user-font-selection.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{image/user-font-selection.png}
  \caption{
  The process of user font selection. (a) Fonts are alphabetically ordered in names. (b) Fonts are embedded in latent space.
  }
%   \Description{}
  \label{fig:user-font-selection}
\end{figure}


==> figure/fig-various-fonts.tex <==
\begin{figure*}[t!]\centering
\includegraphics[width=0.8\linewidth]{image/font-cute,techno,old-english.png}
\caption{
Various fonts tagged as "Cute", "Techno" and "Old English".
} 
% \Description{These fonts are from 1001fonts examples.}
\label{fig:various-fonts}
\end{figure*}



==> figure1.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width = \linewidth]{images/PMnet}
\end{center}
\vspace{-5mm}
\caption{Overview of the proposed method.} 
\vspace{-2mm}
\label{fig:overview}
\end{figure*}

% Overview of the proposed method, which can be trained end-to-end.
% Then the target pose $p_{1:T}^B$ and the target movement $v_{1:T}^B$ are obtained from $p_{1:T}^A$ and $v_{1:T}^A$ separately.
% Then $p_{1:T}^A$ and $v_{1:T}^A$ are retargeted to the target pose $p_{1:T}^B$ and the target movement $v_{1:T}^B$ separately.


% where $p_{1:T}^A$ means the relative coordinates from the root joint position and $v_{1:T}^A$ means the velocity of the root joint
% We decompose the input motion $x_{1:T}^A$ into the frame-by-frame pose $p_{1:T}^A$ and the overall movement $v_{1:T}^A$. Then $p_{1:T}^A$ and $v_{1:T}^A$ are retargeted to the target pose $p_{1:T}^B$ and the target movement $v_{1:T}^B$ respectively.

==> figure2.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[width = \linewidth]{images/figure2}
% \rule{0.99\linewidth}{11cm}
\end{center}
\vspace{-3mm}
\caption{Qualitative comparisons. We present two motion retargeting results, from Mutant to Liam (left) and from Big Vegas to Malcolm (right). The number in orange on the upper left indicates the frame number.}
\label{fig:qualitative}
\vspace{-1mm}
\end{figure*}

% More video results are reported in supplementary material.

==> figure3.tex <==
\begin{figure*}[t!]
\begin{center}
\vspace{-1mm}
\includegraphics[width = \linewidth]{images/figure3_final_final}
% \rule{0.99\linewidth}{3.2cm}
\end{center}
\vspace{-5mm}
\caption{Plots for the overall movement where the horizontal axis represents the frame sequence and the vertical axis represents the corresponding velocity and rotation values. We present the larger plots at \url{https://github.com/ljin0429/PMnet}.}
\label{fig:global}
% \vspace{-3mm}
\end{figure*}

% We present the larger plots in supplementary material.

==> implementation.tex <==




\begin{table}[t!]
\caption{Detailed architecture for $\mathcal{F}_P$, $\mathcal{F}_q$, $\mathcal{F}_{\Delta}$, $\mathcal{F}_M$ and $D$. 
We used the leak rate of 0.2 for leaky ReLU and applied dropout for the whole network with the keep probability of 0.8.
Please visit \url{https://github.com/ljin0429/PMnet} for more details.}
\label{tab:implementation}
% \vspace{-2mm}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Name                    & Layer           & Number of Neurons     & Activation \\
\hline\hline
                        & input           & 66                    & - \\
                        & fc             & 512                   & ReLU \\
$\mathcal{F}_P$         & fc             & 512                   & ReLU \\
                        & fc             & 512                   & ReLU \\
                        & fc             & 512                   & ReLU \\
\hline\hline
$\mathcal{F}_q$         & input           & 512                   & - \\
                        & fc             & 88                    & - \\
\hline\hline
$\mathcal{F}_{\Delta}$  & input           & 512                   & - \\
                        & fc             & 88                    & - \\
\hline
\end{tabular}
\end{center}
\vspace{-3mm}

\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Name                    & Layer           & Kernel      & Stride    & Channel Depth     & Activation  & Length \\
\hline\hline
                        & input         & -           & -         & 4                 & -           & 60 \\
$\mathcal{F}_M$         & 1DConv        & 3           & 1         & 128               & leaky ReLU  & 60 \\
                        & 1DConv        & 3           & 1         & 4                 & -           & 60 \\
\hline\hline
                        & Input           & -           & -         & 3               & -           & 60 \\
                        & 1DConv        & 4           & 2         & 16                & leaky ReLU  & 30 \\
                        & 1DConv        & 4           & 2         & 32                & leaky ReLU  & 15 \\
$D$                     & 1DConv        & 4           & 2         & 64                & leaky ReLU  & 8 \\
                        & 1DConv        & 4           & 2         & 128               & leaky ReLU  & 4 \\
                        & 1DConv        & 4           & 2         & 1                 & -           & 1 \\
                        & output          & -           & -         & 1               & sigmoid     & 1 \\                        
\hline
\end{tabular}
\end{center}
% \vspace{-2mm}
\end{table}


% \begin{table}[t!]
% \caption{Detailed architecture for $\mathcal{F}_M$ and $D$.}
% \label{tab:movement}
% \vspace{-2mm}
% \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Name                    & Layer           & Kernel      & Stride    & Channel Depth     & Activation  & Length \\
% \hline\hline
%                         & input         & -           & -         & 4                 & -           & 60 \\
% $\mathcal{F}_M$         & 1DConv        & 3           & 1         & 128               & leaky ReLU  & 60 \\
%                         & 1DConv        & 3           & 1         & 4                 & -           & 60 \\
% \hline\hline
%                         & Input           & -           & -         & 3               & -           & 60 \\
%                         & 1DConv        & 4           & 2         & 16                & leaky ReLU  & 30 \\
%                         & 1DConv        & 4           & 2         & 32                & leaky ReLU  & 15 \\
% $D$                     & 1DConv        & 4           & 2         & 64                & leaky ReLU  & 8 \\
%                         & 1DConv        & 4           & 2         & 128               & leaky ReLU  & 4 \\
%                         & 1DConv        & 4           & 2         & 1                 & -           & 1 \\
%                         & output          & -           & -         & 1               & sigmoid     & 1 \\                        
% \hline
% \end{tabular}
% \end{center}
% \vspace{-5mm}
% \end{table}


==> result_table.tex <==
\begin{table}[t!]
\caption{Quantitative results on Mixamo dataset~\cite{Mixamo}. For the NKN results, the numbers on the left are the results of our experiments using the code provided from the authors, and the numbers in brackets indicate the performance reported in their paper.}
\label{tab:quantitative}
\vspace{-1mm}
\small
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Method                                          & MSE                        & Notes \\
\hline\hline
                                                & 10.50 (10.25)              & Auto-Encoder \\
NKN (CVPR'18)~\cite{villegas2018neural}         & \textbf{7.68} (8.51)       & Cycle loss \\
                                                & 8.87 (\textbf{7.10})       & Cycle + Adv loss\\
\hline
\hline
Copy                            & 9.00                   & Copy input quaternions and velocities \\
\hline
\hline
\textit{wPP}-PMnet              & 2.54                   & without $\mathcal{L}_{pose}$ \\
\textit{wM}-PMnet               & 2.79                   & without $\mathcal{L}_{motion}$ \\
\textit{wR}-PMnet               & 2.99                   & without $\mathcal{L}_{recon}$ \\
\textit{eqR}-PMnet              & 2.15                   & equal weights for $\mathcal{L}_{recon}$ \\
\hline
\textbf{PMnet}                  & \textbf{1.95}          & Ours \\
\hline
\end{tabular}
\end{center}
\end{table}


% \textit{baseline}-PMnet         & -.--                   & without $\mathcal{L}_{pose}$ and $\mathcal{L}_{motion}$ \\


==> table/tab-cross-data-validation-and-test.tex <==
% \begin{table*}
% \centering
% \caption{Font embedding methods performance comparison with retrieval accuracy. Cross data validation and test results.}
% \label{t4}
% \begin{tabular}{c|cc|cc}
% \noalign{\smallskip}\noalign{\smallskip}\hline\hline
% \multirow{2}{*}{} & \multicolumn{2}{c|}{Trained on Donovan} & \multicolumn{2}{c}{Trained on OFL} \\
% \cline{2-5}
%       & Validation on Donovan  & Test on OFL & Valdiation on OFL & Test on Donovan \\
% \hline
% Font Classification & - & - & - & - \\
%  Font Classification$^{\diamond}$ & - & - & - & - \\
%  Glyph Autoencoder & - & - & - & - \\
%  Glyph Autoencoder$^{\diamond}$ & - & - & - & - \\
%  Two-glyph learning & - & - & - & - \\
% Two-glyph learning$^{\diamond}$ & - & - & - & - \\
% \hline
% \hline
% \end{tabular}
% \end{table*}

\begin{table*}
\centering
\caption{Font embedding methods performance comparison with retrieval accuracy. Cross data validation and test results.}
\label{t4}
\begin{tabular}{c|cc|cc|ccc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multirow{2}{*}{} 
% & \multicolumn{2}{c|}{Trained on Donovan (a\textasciitilde Z)} 
& \multicolumn{2}{c|}{Donovan trainset} 
& \multicolumn{2}{c|}{Donovan trainset + attribute} 
& \multicolumn{3}{c}{OFL trainset} \\
\cline{2-8}
      & Donovan valset
      & OFL testset
      & Donovan valset
      & OFL testset
      & OFL valset
      & OFL testset
      & Donovan valset \\      
\hline
%  Font Classification & 86.12 & - & 87.56 & - & - & - \\
%  Glyph Autoencoder & - & - & - & - & - & - \\
%  Two-glyph learning & 90.89 & - & 91.42 & - & - & - \\
 
 
 Font Classification & 82.17  & 74.86 & 83.11  & 77.08 & 75.30 & 86.82 & 70.3 \\
 Glyph Autoencoder & 25.49 & - & - & - & - & - & - \\
 \rev{Conditional Autoencoder} & 40.84 & 34.88 & - & - & - & - & - \\
 Attr2Font~\cite{WangSIGGRAPH2020} & - & - & 10.40 & 14.17 & - & - & - \\
 Two-glyph learning & 87.11 & 80.31 & 88.45 & 82.27 & 82.80 & 94.69 & 74.01 \\
%   Font Classification & 82.17  & 54.44 & 83.11  & 55.77 & - & - & - \\
%  Glyph Autoencoder & - & - & - & - & - & - & - \\
%  Attr2Font~\cite{WangSIGGRAPH2020} & - & - & - & - & - & - & - \\
%  Two-glyph learning & 87.11 & 57.27 & 88.45 & 61.07 & - & - & - \\
 
 
\hline
\hline
\end{tabular}
\end{table*}

==> table/tab-donovan-dataset.tex <==
% \begin{table*}
% \centering
% \caption{Font embedding methods performance comparison with retrieval accuracy. Cross data validation and test results.}
% \label{t4}
% \begin{tabular}{c|cc|cc}
% \noalign{\smallskip}\noalign{\smallskip}\hline\hline
% \multirow{2}{*}{} & \multicolumn{2}{c|}{Trained on Donovan} & \multicolumn{2}{c}{Trained on OFL} \\
% \cline{2-5}
%       & Validation on Donovan  & Test on OFL & Valdiation on OFL & Test on Donovan \\
% \hline
% Font Classification & - & - & - & - \\
%  Font Classification$^{\diamond}$ & - & - & - & - \\
%  Glyph Autoencoder & - & - & - & - \\
%  Glyph Autoencoder$^{\diamond}$ & - & - & - & - \\
%  Two-glyph learning & - & - & - & - \\
% Two-glyph learning$^{\diamond}$ & - & - & - & - \\
% \hline
% \hline
% \end{tabular}
% \end{table*}

\begin{table}
\centering
\caption{Donovan dataset.}
% \label{tab:unseen-fonts-donovan}
\begin{tabular}{c|c|c}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multirow{2}{*}{} 
% & \multicolumn{2}{c|}{Trained on Donovan (a\textasciitilde Z)} 
& \multicolumn{2}{c}{Trained on Donovan $\mathbb{C}_\text{a-Z}$} 
% & \multicolumn{2}{c|}{Donovan trainset + attribute} 
\\
\cline{2-3}
      & Donovan valset
      & OFL valset 
      \\      
      &  $\text{Ret\_Acc}(\mathbb{C}_\text{a-Z} ) $
      &  $\text{Ret\_Acc}(\mathbb{C}_\text{a-Z} ) $
      \\            
      
\hline
%  Font Classification & 86.12 & - & 87.56 & - & - & - \\
%  Glyph Autoencoder & - & - & - & - & - & - \\
%  Two-glyph learning & 90.89 & - & 91.42 & - & - & - \\
 
 
 


Two-glyph learning & 89.60 & 64.53 \\
Font Classification & 82.17  & 56.56 \\
Font Style Transfer & 71.84 & 38.77 \\
Glyph Autoencoder & 27.13 & 13.96 \\

\hline

\multirow{2}{*}{} 
% & \multicolumn{2}{c|}{Trained on Donovan (a\textasciitilde Z)} 
% & \multicolumn{2}{c}{Donovan trainset} 
& \multicolumn{2}{c}{+ font attributes $\mathbb{A}$} 
\\
\cline{2-3}
      & Donovan valset
      & OFL valset
      \\      
      &  $\text{Ret\_Acc}(\mathbb{C}_\text{a-Z} ) $
      &  $\text{Ret\_Acc}(\mathbb{C}_\text{a-Z} ) $
      \\                
\hline

 Two-glyph learning  & 89.91 & 66.46 \\
 Font Classification  & 83.11  & 58.56 \\
 Font Style Transfer  & 76.71 & 36.71 \\
 Glyph Autoencoder  & 57.87 & 31.97 \\
 
%  Attr2Font~\cite{WangSIGGRAPH2020}  & 10.40 & 14.17 \\
 

 
 
\hline
\hline
\end{tabular}
\end{table}

==> table/tab-donovan-downstream-font-style-transfer.tex <==


\begin{table}
\centering
\caption{Font Style Transfer performance on the O'Donovan dataset with different initial weights.}
\label{tab:donovan-downstream-font-style-transfer}
\begin{tabular}{c|c}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multirow{2}{*}{Font Style Transfer trained on O'Donovan $\mathbb{C}_\text{a-Z} $} 
      & O'Donovan valset 
      \\
      & L1-error
      \\                  
\hline

%  Paired-glyph learning  &  -  \\
%  Font Classification    &  -  \\
%  Font Style Transfer    &  -  \\
 Pretrained {\it Paired-glyph learning} on OFL      &  0.1026  \\
 Pretrained {\it Font Classification} on OFL        &  0.1101  \\
 Pretrained {\it Font Style Transfer} on OFL        &  0.1092  \\
 Pretrained {\it Glyph Autoencoder} on OFL          &  0.1111  \\
 Random Initialization ($\texttt{feat\_dim=1024}$)   &  0.1116  \\
 Random Initialization ($\texttt{feat\_dim=512}$)   &  0.1116  \\
 
 
\hline
\hline
\end{tabular}
\end{table}

==> table/tab-method-comparison.tex <==
\begin{table}
\centering
\caption{Font embedding methods performance comparison with retrieval accuracy}
\label{t3}
\begin{tabular}{c|ccc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
& uppercases & all cases \\
\hline
Font Classification & - & -  \\
Font Attribute Classification & - & -  \\
Glyph Autoencoder  & - & - \\
Glyph-Set Autoencoder  & - & - \\
Two-glyph learning(명칭생각)  & 90.89 & - \\
\hline
\hline
\end{tabular}
\end{table}
\label{tab:method-comparison}

==> table/tab-zero-shot-embedding.tex <==
\begin{table*}
\centering
\caption{Results of retrieval accuracy on unseen characters.}
\label{t4}
\begin{tabular}{c|cc|cc|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
\multirow{2}{*}{} 
% & \multicolumn{2}{c|}{Trained on Donovan (a\textasciitilde Z)} 
& \multicolumn{6}{c}{Trained on Donovan (a\textasciitilde Z)} \\
\hline
& \multicolumn{2}{c|}{Donovan trainset} 
& \multicolumn{2}{c|}{Donovan valset} 
& \multicolumn{2}{c}{OFL testset} \\
\cline{2-7}
      & (0\textasciitilde 9) $\rightarrow$ (a\textasciitilde Z) 
      & (a\textasciitilde Z) $\rightarrow$  (0\textasciitilde 9) 
      & (0\textasciitilde 9) $\rightarrow$ (a\textasciitilde Z) 
      & (a\textasciitilde Z) $\rightarrow$  (0\textasciitilde 9) 
      & (0\textasciitilde 9) $\rightarrow$ (a\textasciitilde Z) 
      & (a\textasciitilde Z) $\rightarrow$  (0\textasciitilde 9) \\      
\hline
 Font Classification & - & - & 67.84 & 71.93 & 60.53 & 68.81 \\
 Font Classification + Attr & - & - & 67.96 & 71.41 & 65.28 & 67.30 \\
 Glyph Autoencoder & - & - & - & - & - & - \\
 Conditional Autoencoder & - & - & 32.68  & 31.86 & 28.26 & 31.72 \\
 Attr2Font~\cite{WangSIGGRAPH2020} & - & - & 10.03 & 9.70 & 11.92 & 13.57 \\
 Two-glyph learning  & - & - & 63.19 & 71.33 & 58.37 & 71.57 \\
 Two-glyph learning + Attr  & - & - & 63.51 & 74.46 & 61.82 & 71.21 \\
\hline
\hline
& \multicolumn{6}{c}{Trained on OFL (a\textasciitilde Z)} \\
\hline
& \multicolumn{2}{c|}{OFL testset} 
& \multicolumn{2}{c|}{Donovan valset} 
& \multicolumn{2}{c}{Multi-language} \\
\cline{2-7}
      & (0\textasciitilde 9) $\rightarrow$ (a\textasciitilde Z) 
      & (a\textasciitilde Z) $\rightarrow$  (0\textasciitilde 9) 
      & (0\textasciitilde 9) $\rightarrow$ (a\textasciitilde Z) 
      & (a\textasciitilde Z) $\rightarrow$  (0\textasciitilde 9) 
      & Korean 
      & Chinese \\      
\hline
 Font Classification & 58.56 & 66.60 & 55.37 & 56.06 & - & - \\
 Glyph Autoencoder & - & - & - & - & - & - \\
 Two-glyph learning & 60.59 & 69.48 & 56.41 & 61.08 & - & - \\
\hline
\hline
\end{tabular}
\end{table*}

==> temp.tex <==

\section{Guidelines}
\label{sec:intro}
From 2009, the proceedings of BMVC (the British Machine Vision
Conference) will be published only in electronic form.  This document
illustrates the required paper format, and includes guidelines on
preparation of submissions.  Papers which fail to adhere to these
requirements may be rejected at any stage in the review process.

\LaTeX\ users should use this template in order to prepare their paper.
Users of other packages should emulate the style and layout of this
example.  Note that best results will be achieved using {\tt pdflatex},
which is available in most modern distributions.

\subsection{Paper length}
Papers must be 9~pages in length, {\em excluding} the bibliography.
%Length is counted from the bottom of the title on the first page.  Therefore, the
%bibliography should begin eight lines into page ten.  This is an
%approximate measure, intended to encourage brevity, but authors should keep
%in mind that blatant disregard of this instruction will cause reviewers to
%require greater originality and impact of the submission.
{\bf Papers which are
clearly overlength will not be reviewed}.  This includes papers where the
margins and formatting are deemed to have been significantly altered from
those laid down by this style guide.  The reason such papers will not be
reviewed is that there is no provision for supervised revisions of
manuscripts.  The reviewing process cannot determine the suitability of the
paper for presentation in nine pages if it is reviewed in twelve.

The bibliography should begin immediately after the paper text.  It may
be of any length, within reason.  It should {\em not} include
annotations, figures, or any other paraphernalia intended to subvert the
paper length requirement.


\begin{figure}
\begin{tabular}{ccc}
\bmvaHangBox{\fbox{\parbox{2.7cm}{~\\[2.8mm]
\rule{0pt}{1ex}\hspace{2.24mm}\includegraphics[width=2.33cm]{images/eg1_largeprint.png}\\[-0.1pt]}}}&
\bmvaHangBox{\fbox{\includegraphics[width=2.8cm]{images/eg1_largeprint.png}}}&
\bmvaHangBox{\fbox{\includegraphics[width=5.6cm]{images/eg1_2up.png}}}\\
(a)&(b)&(c)
\end{tabular}
\caption{It is often a good idea for the first figure to attempt to
encapsulate the article, complementing the abstract.  This figure illustrates
the various print and on-screen layouts for which this paper format has
been optimized: (a) traditional BMVC print format; (b) on-screen
single-column format, or large-print paper; (c) full-screen two column, or
2-up printing. }
\label{fig:teaser}
\end{figure}

\subsection{Dual submission}
By submitting this manuscript to BMVC, the authors assert that it has not
been previously published in substantially similar form, and no paper
currently under submission to a conference contains significant overlap
with this one.  If you are in doubt about the amount of overlap, cite the
dual submission (as described below), and argue in the body of your paper
why this is a nontrivial advance.  A simultaneous journal submission would
be expected to have significant additional material not in the conference
paper, and should not be previously published, nor in the final acceptance
stages. The conference chairs reserve the right to cancel
submission of any paper which is found to violate these conditions.  In
particular, {\em uncited} dual submissions will be summarily dealt with.

\subsection{Anonymity and blind review}
BMVC operates a double-blind review process.  Your review submission {\bf
must not identify you as the author}.  This means, in particular, that the
author list should be replaced by the words ``BMVC {\em YYYY} Submission \#
{\em NNN}'', where the italics are to indicate the year and the submission
number.  The provided \LaTeX\ command \verb'\bmvcreviewcopy' does this
automatically.  In addition, acknowledgements should not be included in the
review copy.

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review {\bf does not mean that one must remove
citations to one's own work}---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  That is all.  (But see below for
techreports)

Saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith, it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an excellent paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you will almost certainly
need to refer to that submission in order to explain the differences,
just as you would if you or others had previously published related
work.  In such cases, include the anonymized parallel
submission~\cite{Authors06} as additional material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', ECCV 2006 Submission ID 324,
Supplied as additional material {\tt eccv06.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors06b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the ICLL'70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.

FAQ: Are acknowledgements OK?  No.  Leave them for the final copy.

\subsection{Citations}
When citing a multi-author paper, you may save space by using ``{\em et
alia}'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is
a complete word.)  The provided \verb'\etal' macro is a useful {\em aide
memoire} in this regard.  However, use it only when there are three or more
authors.  Thus, the following is correct: `` Frobnication has been trendy
lately.  It was introduced by Alpher~\cite{Alpher02}, and subsequently
developed by Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher
\etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

%For this citation style, keep multiple citations in numerical (not
%chronological) order, so prefer
We use {\tt natbib}, so citations in random order are nicely sorted:
 \cite{Alpher03,Alpher02,Authors06b,Authors06}.  However, we don't use the
compress option, as we want each reference to have its own hyperlink and
popup window.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may remove
the \verb'[review]' option from the \verb'\documentclass' statement.)
Reviewers: note that the ruler measurements do not align well with lines
in the paper --- this turns out to be very difficult to do well when the
paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (e.g.\ this line is $210.5$), although in
most cases one would expect that the approximate location ($210$ in the
previous example) will be adequate.


\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description~\cite{Mermin89} of how to write mathematics.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors06}.  Where appropriate, include the name(s) of
editors of referenced books.


%------------------------------------------------------------------------
\subsection{Color}

Color is valuable, and will be visible to readers of the electronic copy.
However ensure that, when printed on a monochrome printer, no important
information is lost by the conversion to grayscale.

